Tighter expected generalization error bounds via Wasserstein distance

This work presents several expected generalization error bounds based on the Wasserstein distance. More specifically, it introduces full-dataset, single-letter, and random-subset bounds, and their analogues in the randomized subsample setting from Steinke and Zakynthinou [1]. Moreover, when the loss function is bounded and the geometry of the space is ignored by the choice of the metric in the Wasserstein distance, these bounds recover from below (and thus, are tighter than) current bounds based on the relative entropy. In particular, they generate new, non-vacuous bounds based on the relative entropy. Therefore, these results can be seen as a bridge between works that account for the geometry of the hypothesis space and those based on the relative entropy, which is agnostic to such geometry. Furthermore, it is shown how to produce various new bounds based on different information measures (e.g., the lautum information or several $f$-divergences) based on these bounds and how to derive similar bounds with respect to the backward channel using the presented proof techniques.

==> NeurIPS 2021 - Tighter Expected Generalization Error Bounds via Wasserstein Distance (copy)/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Color codes for comments
\definecolor{orange}{rgb}{1,0.4,0.0}
\newcommand{\rt}[1]{\textbf{\textcolor{red}{{#1}}}}
\newcommand{\ms}[1]{\textbf{\textcolor{olive}{{#1}}}}
\newcommand{\gb}[1]{\textbf{\textcolor{brown}{{#1}}}}
\newcommand{\brg}[1]{{\textcolor{orange}{{#1}}}}
\newcommand{\rev}[1]{{\textcolor{black}{{#1}}}}


%% KL divergence command
% Usage: \KL{f}{g} or \KL[\bigg]{f}{g}
\DeclarePairedDelimiterXPP{\KL}[2]{D_\textnormal{KL}}{(}{)}{}{%
#1\:\delimsize\|\:#2% 
}

%% Renyi divergence command
% Usage: \RD{f}{g} or \RD[\bigg]{f}{g}
\DeclarePairedDelimiterXPP{\RD}[2]{D_{\alpha}}{(}{)}{}{%
#1\:\delimsize\|\:#2%
}

%% Probability with optional conditioning
% Usage: \Prob{A \given B} or \Prob{A}
\DeclarePairedDelimiterXPP\Prob[1]{\mathbb{P}}{\lbrace}{\rbrace}{}{
\newcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}


%% L-norm
% Usage: \lnorm{x}{2} -> ||x||_2
\DeclarePairedDelimiterXPP{\lnorm}[2]{}{\lVert}{\rVert}{_{#2}}{#1}

%% Shortcuts for Algorithm, Expectation, and Real numbers
\newcommand{\bA}{\ensuremath{\mathbb{A}}}
\newcommand{\bE}{\ensuremath{\mathbb{E}}}
\newcommand{\bR}{\ensuremath{\mathbb{R}}}
\newcommand{\bN}{\ensuremath{\mathbb{N}}}
\newcommand{\bP}{\ensuremath{\mathbb{P}}}
\newcommand{\bI}{\ensuremath{\mathbbm{1}}}
\newcommand{\bW}{\ensuremath{\mathbb{W}}}

%% Shortcuts for calligraphic S, T, W, X, Y, and Z
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cL}{\ensuremath{\mathscr{L}}}

%% Shortcut for stacking something in a math equation (e.g., in a '=')
% Usage: \stack{(a)}{=}
\newcommand{\stack}[2]{\stackrel{\mathclap{(#1)}}{#2}}

%% Command for probability independence
\newcommand{\indep}{ {\perp\!\!\!\perp} }

%% Command for Q.E.D. since amsthm cannot be loaded for JMLR
%\newcommand{\qedsymbol}{$\square$}
%\newcommand{\qedsymbol}{\jmlrQED}

\usepackage[style=0,ntheorem]{mdframed}
    \mdfsetup{%
    topline=false,
    rightline=false,
    bottomline=false,
    linewidth=1.2pt,
    innerleftmargin=2pt,
    innerrightmargin=0pt,
    skipabove=0.1\baselineskip,
}

\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
\newtheorem{claim}{Claim}
\newmdtheoremenv{proposition}{Proposition}
\newtheorem{notation}{Notation}
\newmdtheoremenv{theorem}{Theorem}
\newmdtheoremenv{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newmdtheoremenv{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
